The Dark Machines Anomaly Score Challenge: Benchmark Data and Model Independent Event Classification for the Large Hadron Collider

We describe the outcome of a data challenge conducted as part of the Dark Machines Initiative and the Les Houches 2019 workshop on Physics at TeV colliders. The challenged aims at detecting signals of new physics at the LHC using unsupervised machine learning algorithms. First, we propose how an anomaly score could be implemented to define model-independent signal regions in LHC searches. We define and describe a large benchmark dataset, consisting of >1 Billion simulated LHC events corresponding to $10~\rm{fb}^{-1}$ of proton-proton collisions at a center-of-mass energy of 13 TeV. We then review a wide range of anomaly detection and density estimation algorithms, developed in the context of the data challenge, and we measure their performance in a set of realistic analysis environments. We draw a number of useful conclusions that will aid the development of unsupervised new physics searches during the third run of the LHC, and provide our benchmark dataset for future studies at https://www.phenoMLdata.org. Code to reproduce the analysis is provided at https://github.com/bostdiek/DarkMachines-UnsupervisedChallenge.

==> glossary.tex <==
\newglossaryentry{SM}
{
    name = Standard Model,
    description = {The model describing the dynamics and interactions of all known particles, in terms of quantum fields and symmetries. }
}
 
 
\newglossaryentry{QCD}
{
    name = Quantum Chromo-Dynamics (QCD),
    description = {The subset of the Standard Model describing the subnuclear strong force.}
}
 
\newglossaryentry{fourmom}
{
    name = 4-momentum,
    description = {The 4-dimensional vector describing energy $E$ and 3-dimensional momentum of a particle: $(E,\vec{p})=(E, p_x, p_y, p_z)$. }
}


\newglossaryentry{jet}
{
    name = Jet,
    description = {Quarks cannot exist on their own, and must combine to form hadrons, subatomic particles of two or more quarks which are bound together by the strong force. This process of forming hadrons is called hadronisation. A jet is a cone of hadrons that have been formed due to the hadronisation of quarks and gluons produced during the collisions in the LHC.}
}
 
\newglossaryentry{pt}
{
    name = Transverse momentum ($p_T$),
    description = {}
}

\newglossaryentry{xsec}
{
    name = Cross section,
    description = {}
}

\newglossaryentry{lumi}
{
    name = Luminosity,
    description = {}
}

\newglossaryentry{schannel}
{
    name = s-channel,
    description = {A scattering process where...}
}

\newglossaryentry{tchannel}
{
    name = t-channel,
    description = {}
}

\newglossaryentry{newphysics}
{
    name = New Physics,
    description = {The unknown physics lying beyond the Standard Model. }
}

\newglossaryentry{eta}
{
    name = Pseudo-rapidity ($\eta$),
    description = {In cylindrical coordinates,
    where $\hat z$ axis coincides with the protons beam line, 
    and the angular variables $\theta, \phi$ map the detector barrel, 
    the pseudo-rapidity is defined as $\eta \equiv-\ln\tan (\theta/2)$, 
    where $-\infty<\eta<+\infty$ for $\pi\geq \theta\geq 0$ (e.g. $\eta=0$ for
    $\theta=\pi/2$, and $\eta=+\infty$ for $\theta=0$).
    }
}

\newglossaryentry{phi}
{
    name = Azimuthal angle ($\phi$),
    description = {In cylindrical coordinates,
    where $\hat z$ axis coincides with the protons beam line, 
    and the angular variables $\theta, \phi$ map the detector barrel, 
    $\phi$ is the azimuthal angle.}
}

\newglossaryentry{gev}
{
    name = GeV,
    description = {Giga-ElectronVolts,
    corresponding to $10^9$ eV.}
}

